Deep learning for scene recognition from visual data: a survey

The use of deep learning techniques has exploded during the last few years, resulting in a direct contribution to the field of artificial intelligence. This work aims to be a review of the state-of-the-art in scene recognition with deep learning models from visual data. Scene recognition is still an emerging field in computer vision, which has been addressed from a single image and dynamic image perspective. We first give an overview of available datasets for image and video scene recognition. Later, we describe ensemble techniques introduced by research papers in the field. Finally, we give some remarks on our findings and discuss what we consider challenges in the field and future lines of research. This paper aims to be a future guide for model selection for the task of scene recognition.

==> x_Analysis.tex <==
\section{Performance Analysis}\label{sec:discussion}

The proposed methods are considered quantitatively, by judging their performances based on metrics such as accuracy (top-1 and top-5), as well as qualitatively, by analysing their performances and limitations in the context of the evaluated datasets. The implementation and the results achieved by the approaches cannot be judged independent of their experimental setup (i.e. dataset, architecture of the CNN), therefore the scope and limitations of the conducted experiments must also be considered.

% quantitative (accuracy)

The quantitative comparison refers to the top-1 accuracy metric, which is defined as the percentage of total correct predictions out of the total number of data points in the test set. 

\subsection*{Generalization of Places365 (?)}
The method described in Section \ref{subsec: places} (places CNN) displayed the highest accuracy, 92.99\%, on the SUN Attribute dataset \cite{sun_attribute} (used as a test set in this case). The architecture which obtained this score is VGG \cite{vgg16}, pre-trained on the Places365 dataset. The method described in Section \ref{subsec:obj+places} (object and places CNN) obtained the highest accuracy of 95.18\% on the 15 scenes dataset \cite{15_scenes} with the dual hybrid architecture proposed (two-scale model consisting of ImageNet and Places pre-trained networks based on the scale). Considering the study presented by \cite{sun_database}, both approaches obtain a significantly higher accuracy in contrast to a human expert which only achieves a percentage of 70.60\% in accuracy.

To compare the performance of the above approaches for static scene recognition, their performance on the following datasets is considered: 15 scenes dataset \cite{15_scenes}, MIT Indoor 67 \cite{mitindoor67} and SUN 397 \cite{sun397}. An overview of the quantitative results comparison is presented in Table \ref{tab:res_overview}.

\begin{table}
\centering
    \begin{tabular}{l l l l}
    & 15 scenes & MIT Indoor & SUN 397  \\
    \hline \hline
    \multicolumn{4}{c}{ \textit{Places CNNs}}  \\
    \hline
    Places365 AlexNet & 89.25\% & 70.72\% & 56.12\%   \\
    Places365 GoogleNet & 91.25\%  & 73.20\%  & 58.37\%   \\
    Places365 VGG & 91.97\%  & 76.53\%  & \textbf{63.24\%}   \\
    Hybrid1365 VGG & \textbf{92.15\%}  & \textbf{79.49\%}  & 61.77\%   \\
    \hline \hline
    \multicolumn{4}{c}{ \textit{Object and scene centric knowledge at scale} }  \\
    \hline
    7-scale Hybrid VGG & \textbf{94.08\%}  & 80.22\%  (w/ FT) & 63.19\%*   \\
    7-scale Hybrid AlexNet & 93.90\%  & \textbf{80.97\%}  (w/ FT) & \textbf{65.38\%}   \\
    \end{tabular}
    \caption{An overview of the quantitative comparison between methods proposed in \cite{places365} and \cite{objects_scenes_scale}. The winning performances are highlighted in bold; w/FT refers to the fine-tuning of the architecture on the corresponding dataset.
    *6 scales only, scale 1827x1827 not included due to the nature of the dataset.}
    \label{tab:res_overview}
\end{table}

Moreover, the Hybrid1365 VGG architecture scores the highest average accuracy of 81.48\% over all the experiments conducted for the place-centric CNN approach (has highest performance for 2 out of 3 comparison datasets as shown in Table \ref{tab:res_overview}). This, together with the quantitative comparison above, shows that the approach of combining both object-centric and scene-centric knowledge can potentially establish a new performance standard for scene recognition.

The results achieved by the T-ResNet architecture described in Section \ref{subsec:dynamic} will be presented individually, since there are no grounds for comparison with the previously mentioned methods due to the different characteristics of the corresponding data (static vs. dynamic). The YUP++ dataset \cite{dynamic_scenes} was used for proving the performance of the novel T-ResNet model. T-ResNet is mainly compared with the classical ResNet architecture as shown in Table \ref{tab:results_dynamic}. The superiority of the T-ResNet is evident: T-ResNet achieves the following percentages in accuracy: 92.41\% on the YUP++ static camera partition, 81.50\% on the YUP++ moving camera partition and finally 89.00\% on the entire YUP++ dataset. Oppositely, ResNet achieves the respective percentages: 86.50\%, 73.50\% and 85.90\%. The most significant difference worth of 8 percentage points is attained for the moving camera partition of the dataset, which presents a more complex challenge (in comparison with the dynamic data captured with a static camera). This demonstrates the superiority of the spatio-temporal approach. 

\begin{table}[]
    \centering
    \begin{tabular}{l l l l}
         & YUP++ static & YUP++ moving & YUP++ complete \\
         \hline \hline
         \multicolumn{4}{c}{\textit{Temporal residual network for dynamic scenes}}\\
         \hline
        ResNet & 86.50\% & 73.50\% & 85.90\% \\
        T-ResNet & \textbf{92.41\%} & \textbf{81.50\%} & \textbf{89.00\%}
    \end{tabular}
    \caption{Overview of the results achieved by the spatio-temporal residual network (T-ResNet) proposed in \cite{dynamic_scenes}.}
    \label{tab:results_dynamic}
\end{table}
% qualitative (datasets, examples, limitations, biased)

\subsection{Qualitative comparison of the presented methodology}
\textcolor{blue}{is this a qualitative analysis or a generalization capability analysis? to check }

Addressing the task of scene recognition from the place perspective as presented in Section \ref{subsec: places}, the CNNs are expected to learn deep features that are relevant for the contextual clues present in the image. Literature \cite{places365} observers that the low-level convolutional layers detect low-level visual concepts such as object edges and textures, while the high-level layers activate on entire objects and scene parts. Even though the model has been previously trained on an exclusively places-centric dataset, the network still identifies semantic clues in the image by detecting objects alongside contextual clues. Therefore, CNNs trained on the Places Database (which does not contain object labels) could still be employed for object detection. 

% Object detectors emerge as an intermediate state of the place trained networks,

Another aspect arising from training the same architecture on datasets with different number of scene categories (i.e. Places205 and Places365) proves that having more categories leads to better results as well as more predicted categories. We can observe that the architecture AlexNet trained on Places205 obtains 0.572 top-1 accuracy, while the same architecture trained on Places365 obtains 0.577 accuracy. For the places CNN approach two main types of miss-classifications occur (see Figure \ref{fig:places_misclass}): on one hand, less-typical activities happening in a scene context (e.g. taking a photo at a construction site) and on the other hand, images depicting multiple scene parts. A possible solution, as proposed by \cite{places365}, would represent assigning multiple ground-truth labels in order to capture the content of an image more precisely.


\begin{comment}
\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{images/qualitative_places.png}
    \caption{Examples of validation set mis-classifications of the Places365-VGG architecture proposed by \cite{places365}. The ground truth label is referred to as GT. It can be observed that the top-5 predictions are, to some extent, related to the GT category, which would suggest introducing multi-label GTs.}
    \label{fig:places_misclass}
\end{figure}
\end{comment}


%qualitative dynamic
The T-ResNet architecture, alongside the corresponding introduced dataset, established a new benchmark in the sub-field of dynamic scene recognition. The dataset introduced in \cite{dynamic_scenes} poses new challenges by introducing a larger variety of classes (i.e. 20 classes as compared to the previously largest dataset which contains only 16 classes) together with more complex data (i.e. videos with camera motion). T-ResNet obtains state-of-the art results, as per literature \cite{dynamic_scenes}, for the scenes captured by a static camera; the model exhibits strong performance for classes with linear motion patterns (for example, classes 'elevator', 'ocean', 'windmill farm'), however, for scene categories presenting irregular or mixed defining motion patterns (for example, classes 'snowing' and 'fireworks') the performance is negatively impacted. The authors of \cite{dynamic_scenes} observed that, for data points which contain camera motion, T-ResNet presents a decrement in performance. The proposed model exhibits difficulties distinguishing intrinsic scene dynamics from the additional motion of the camera. Further research is required to account for this difference.

The results achieved by the T-ResNet model illustrate the potential of spatio-temporal networks for dynamic scenes. The transformation from a purely spatial network to a spatio-temporal one can succeed on the basis of a very small training set (i.e. only 10\% of the YUP++ dataset introduced) as proven by \cite{dynamic_scenes}. Well-initialized spatial networks can be efficiently transformed to extract spatio-temporal features, therefore, in theory every network that performs well on static scenes could be easily adapted to dynamic scenes. 


The authors of \cite{dynamic_scenes} conducted experiments to analyse the generalization ability of the proposed network on action recognition tasks. For the challenge of action recognition, optical flow is a discriminative feature. The proposed T-ResNet architecture presents a healthy performance improvement on two popular action recognition datasets (i.e. UCF101 \cite{ucf101}, HMDB51 \cite{hmdb51}) in contrast to previously achieved state-of-the-art results as shown in Table \ref{tab:t-resnet_qualitative}. The performance boost of T-ResNet, according to \cite{dynamic_scenes}, is based on the added temporal filters which are 1x1 in spatial dimension and span only 3 instances in time, which come at a very low cost.

\begin{table}[]
    \centering
    \begin{tabular}{l l l}
         & UCF101 & HMDB51 \\
    \hline \hline
    &  \textit{State of the art} & \\
        \hline
    Literature \cite{wang_actions} & 92.40\% & 62.00\% \\
    Literature \cite{feichtenhofer_convolutional} & 92.50\% & 65.40\% \\
    Literature \cite{video_action} & 93.40\% & 66.40\% \\
    \hline \hline
    & \textit{T-ResNet \cite{dynamic_scenes}} &\\
    \hline
    Appearance & 85.40\% & 51.30\% \\
    Flow & 89.10\% & 62.00\% \\
    Fusion & \textbf{93.90\%} & \textbf{67.20\%} \\
    \end{tabular}
    \caption{Accuracy comparison of the T-ResNet architecture and state-of-the-art models on action recognition datasets (UCF101 \cite{ucf101}, HMDB51 \cite{hmdb51}) as presented in \cite{dynamic_scenes}. The temporal residual units are applied on the appearance and flow networks of a two-stream architecture \cite{appearance_flow_net}. The fusion of the two streams achieves the highest accuracy. }
    \label{tab:t-resnet_qualitative}
\end{table}

